Evolution of new regulatory functions on biophysically realistic fitness landscapes

Regulatory networks consist of interacting molecules with a high degree of mutual chemical specificity. How can these molecules evolve when their function depends on maintenance of interactions with cognate partners and simultaneous avoidance of deleterious "crosstalk" with non-cognate molecules? Although physical models of molecular interactions provide a framework in which co-evolution of network components can be analyzed, most theoretical studies have focused on the evolution of individual alleles, neglecting the network. In contrast, we study the elementary step in the evolution of gene regulatory networks: duplication of a transcription factor followed by selection for TFs to specialize their inputs as well as the regulation of their downstream genes. We show how to coarse grain the complete, biophysically realistic genotype-phenotype map for this process into macroscopic functional outcomes and quantify the probability of attaining each. We determine which evolutionary and biophysical parameters bias evolutionary trajectories towards fast emergence of new functions and show that this can be greatly facilitated by the availability of "promiscuity-promoting" mutations that affect TF specificity.

==> ModelDescription/BaselineParameters.tex <==
\begin{table}[H]
\begin{tabular}{|c|>{\centering}m{10cm}|c|}
\hline
Parameter & Explanation & Baseline value\tabularnewline
\hline
\hline
$L$ & BS length, length of sequences that TFs bind & $5$\tabularnewline
\hline
$\epsilon$ & Energy contribution per bp towards TF-BS binding & $3\:k_{B}T$\tabularnewline
\hline
$C_{0}$ & Active TF free concentration in the presence of signal, set such that
$p_{jm}=0.5$ at $k=1.5$ & $4.5$\tabularnewline
\hline
$f_{1}$ & Frequency of signal $1$ & $0.5$\tabularnewline
\hline
$f_{2}$ & Frequency of signal $2$ & $0.5$\tabularnewline
\hline
$\rho$ & Correlation between input signals & $0$\tabularnewline
\hline
$\beta_{X}$ & $\beta_{jm}$ when $p_{jm}^{*}=0$ for gene $j$ in environment $m$: penalty
in fitness on activating a gene when it is not needed (crosstalk interaction) & $0.5$\tabularnewline
\hline
other $\beta$ & $\beta_{jm}$ when $p_{jm}^{*}=1$ for gene $j$ in environment $m$: penalty in fitness on not activating a gene when it is needed (functional
interaction) & $1$\tabularnewline
\hline
$Ns$ & Selection strength & $25$\tabularnewline
\hline
$r_{S}$ & Relative mutation rate of the signal sensing domain compared to the
binding site mutation rate per bp & $1$\tabularnewline
\hline
$r_{TF}$ & Relative mutation rate of the TF consensus sequence per bp compared
to the binding site mutation rate per bp & $1$\tabularnewline
\hline
\end{tabular}

\caption{Model parameters and their baseline values. }


\end{table} 
